Learning to Imagine Manipulation Goals for Robot Task Planning

Prospection is an important part of how humans come up with new task plans, but has not been explored in depth in robotics. Predicting multiple task-level is a challenging problem that involves capturing both task semantics and continuous variability over the state of the world. Ideally, we would combine the ability of machine learning to leverage big data for learning the semantics of a task, while using techniques from task planning to reliably generalize to new environment. In this work, we propose a method for learning a model encoding just such a representation for task planning. We learn a neural net that encodes the $k$ most likely outcomes from high level actions from a given world. Our approach creates comprehensible task plans that allow us to predict changes to the environment many time steps into the future. We demonstrate this approach via application to a stacking task in a cluttered environment, where the robot must select between different colored blocks while avoiding obstacles, in order to perform a task. We also show results on a simple navigation task. Our algorithm generates realistic image and pose predictions at multiple points in a given task.

==> discussion.tex <==

There are a few lessons we can take away from these results.

First, using a multiple hypothesis loss allows us to capture stochasticity and variability in robot task plan execution.
Since a task plan may fail, or an object may be grasped in slightly different positions, it makes sense that we execute this differently depending on the exact circumstances.

Second, we specifically come away with a set of lessons for how best to design these networks.

\subsubsection*{Stochasticity}
Capturing randomness is important. Using separate ``transform'' mapping
from the input state to the resulting state gives us crisper, more accurate
output predictions, where each transform encodes a slightly different
possible grasp or approach.

\subsubsection*{Network Training}
Using dropout in either the transforms or in the decoder will blur
the results, giving us a less accurate estimate of what the future world
may look like. Using insufficient dropout will likewise cause issues.

We provide a different random seed at each time step for each prediction; the
networks are able to use this noise during execution to capture some additional
level of uncertainty.


